Machine Learning Across Cultures: Modeling the Adoption of Financial Services for the Poor

Recently, mobile operators in many developing economies have launched "Mobile Money" platforms that deliver basic financial services over the mobile phone network. While many believe that these services can improve the lives of the poor, a consistent difficulty has been identifying individuals most likely to benefit from access to the new technology. Here, we combine terabyte-scale data from three different mobile phone operators from Ghana, Pakistan, and Zambia, to better understand the behavioral determinants of mobile money adoption. Our supervised learning models provide insight into the best predictors of adoption in three very distinct cultures. We find that models fit on one population fail to generalize to another, and in general are highly context-dependent. These findings highlight the need for a nuanced approach to understanding the role and potential of financial services for the poor.

==> conclusion.tex <==
In this paper, we present a new approach to feature engineering that uses DFA to construct a very large number of features from a concise set of rules. By applying this technique on data from three different countries, we are able to show that this approach outshines the traditional approaches for Mobile Money adoption. The analysis also highlights the significant determinants of Mobile Money, such as  network structure in Ghana and Pakistan, and the geographic diversity in Zambia. Our study also makes it clear that not only the country specific models have varied performance but the models trained in one location do not perform well in another. 

==> dfa.tex <==
The Deterministic Finite Automaton described in Section \ref{sec:dfa} is defined in part by a set of transition functions $\delta : Q \times \Sigma \rightarrow Q$ that define the legal transitions between states $Q$:

\begin{itemize}
	\item \textit{Filter}: $Q \times CDR \rightarrow CDR$ \\
				Operations filter the data on the basis of the type of communication (voice, sms) or the direction the activity (incoming, outgoing).
	\item \textit{Map}: $Q \times CDR \rightarrow (field, CDR)$\\
				Operations are similar to `group by' operations, which group the input CDR according to the value of a field in the CDR. All data are initially mapped by ego $i$, creating $N$ subsets of CDR, one corresponding to each individual.
				Other common \textit{map} criteria include alter, location, and day-of-week.
	\item \textit{Select}: $Q \times (field^*,CDR) \rightarrow (field^*,fields)$ \\
				Operations extract a field (or column) from the CDR. Common select criteria are duration, location, and a constant 1 used to count transactions.
	\item \textit{Reduce}: $Q \times (field^*, fields) \rightarrow (field^*, value)$\\
				 Operations `aggregate' a set of values into a single value. Valid operations include unique, count, average, standard deviation, radius of gyration, and entropy. Whether a \textit{reduce} operation is legal depends on the data type of the field to which it is being applied. \textit{Reduce'} is a special operation that aggregates values across all of an ego's alters, creating a feature that represents the \{average, standard deviation\} of the individual's first-degree network.
\end{itemize}	


==> methods.tex <==
The DFA-based process of feature engineering described  above generates thousands of features that quantify patterns of mobile phone use. Using with these features, our goals are to (a) use these features to understand the determinants of Mobile Money use, (b) build a predictive model that can be used to identify likely adopters, and (c) determine the extent to which models and features from one context can generalize to another.




We first use a variety of supervised learning algorithms to a) differentiate between Voice Only subscribers and Registered Mobile Money Users (one or more Mobile Money transactions); second, we attempt to differentiate between Voice Only and Active Mobile Money users (at least one transaction per month). Although we used a bunch of classifiers which are robust to overfitting, we report only the results from gradient boosting\cite{friedman2001greedy}, which outperformed the other classifiers by a small margin. We drew a stratified random sample of 10,000 subscribers from each of the three user type (Voice Only, Registered Mobile Money, Active Mobile Money) from each country. 

Similarly, to highlight the importance of individual features we calculate two metrics namely \textbf{(Unconditional) AUC}   and b) \textbf{(Conditional) Normalized feature importance}. Unconditional AUC is obtained when running a bivariate logistic regression of the user type on each feature separately. Normalized (Conditional) feature importance indicates the {relative} significance of each feature in the final gradient boosting classifier operating on all of the features. 

==> related.tex <==
The literature on the mobile money adoption has been dominated by the macroeconomic and ethnographic work aimed at promoting the adoption of Mobile Money. The macro-scale work is concerned with the national and regulatory forces that can impact the adoption of mobile money. \cite{mas_scaling_2011,dermish_branchless_2011,donovan_mobile_2012}. The ethnographic work has focused primarily on qualitative studies of how mobile money can be integrated into the daily lives of the poor \cite{morawczynski_exploring_2009,mobile_banking_adoption_mehdi,etim2014mobile}.%

The strand of literature that is most closely related to our work contains several papers that use transactions data from mobile operators to study product adoption and churn \cite{sundsoy_big_2014,sundsoy_big_2014, cgap} . Relative to these studies, our study moves this literature forward by (a) innovating in the method used to generate features, thereby providing a systematic and comprehensive approach to feature engineering; (b) leveraging data from three different contexts to calibrate the external validity and generalizability of our results; and (c) carefully articulating the experiments in a way that will enable other researchers to replicate and extend these methods.

==> tabs/cond_features_ghana.tex <==
\begin{table*}[tb]
	\centering
	\begin{tabular}{l*{4}{c}}
		\hline
		\textbf{Registered Mobile Money Feature}& \textbf{Importance}&\textbf{Active Mobile Money Feature}& \textbf{Importance} \\ \hline
		%1
St.Dev. for number of unique days with out sms for mobile money alter &162.0 &Standard Deviation of Network Size for all alter&338.0 \\
Standard Deviation of Network Size for all alter&149.0&Standard Deviation of Network Size for voice alter&258.0\\
Average number of incoming sms locations for mobile money alter&145.0&Average of Network size for voice alter &200.0\\
Average out network size for mobile money alter&108.0&St. Dev. of Outgoing sms network size for voice alter&200.0\\
Average network size for mobile money alter&99.0&Voice Network Location Diversity for all alter &200.0\\
Average Distance between outgoing calls parties for all alter&94.0&Standard Deviation for Active Days for all alter&104.0\\
Average Incoming SMS network size for mobile money alter&92.0&Standard Deviation for no of outcalls and sms for mobile money alter&82.0\\
Average Distance for incoming voice calls for all alter&87.0&Standard Deviation for no of outcalls and sms for mobile money alter&81.0\\
Standard Deviation of Radius of Gyration for Voice Network for voice alter&85.0&Average Network size for mobile money alter& 67\\
Ego's Average Duration for outgoing calls&80.0&standard deviation of Average out call duration for all alter&67.000000\\
		\hline \hline
	\end{tabular}
	\caption{\textbf{Top Features (tested individually).}  Individual features that are most predictive of churn. The ranked list of features is determined by individually assessing the ability of each feature to predict adoption, absent other features.\label{tab:features1}}
\end{table*}

==> tabs/uncond_features_ghana.tex <==
\begin{table*}[tb]
	\centering
	\begin{tabular}{l*{4}{c}}
		\hline
		\textbf{Registered Mobile Money Feature}& \textbf{AUC}&\textbf{Active Mobile Money Feature}& \textbf{AUC} \\ \hline
		%1
		St. Dev. of Voice Only Alter's network size & 0.82 &St. Dev. of the Voice Only Alter's Network Size &	0.82\\ 
		%2
		Average of Voice Only Alter's network size &0.80&Average of the Voice Only Alter's Network Size &	0.80                               \\ 
		%3
		St. Dev. of Voice Only Alter's network size for outgoing activity& 0.77 &St. Dev. of the Voice Only Alter's Activity Count& 0.75                            \\ 
		%4
		Average of Voice Only Alter's network size for outgoing activity& 0.75 &St. Dev. of the Voice Only Alter's Unique Locations Count	& 0.75\\  
		%5
		St. Dev. of the Voice Only Alter's unique  locations & 0.75&St. Dev. of the Voice Only Alter's Outgoing Activity Count& 	0.75                                \\
		%6
		St. Dev. of Voice Only Alter's network size  & 0.75&St. Dev. of the Mobile Money Alter's Outgoing SMS Receiver Cells	& 0.75\\ 
		%7
		St. Dev. of Voice Only Alter's network size for outgoing activity    & 0.75&St. Dev. of the Mobile Money Alter's No of Days with outgoing SMS	&0.75                                \\ 
		%8
		St. Dev. of Voice Only Alter's active days & 0.75& St. Dev. of the Mobile Money Alter's No of Cells from which SMS was received	&0.75                               \\ 
		%9
		St. Dev. of Voice Only Alter's incoming transactions  & 0.72&St. Dev. of the Mobile Money Alter's Incoming SMS Network Size&	0.75                                \\
		%10
		St. Dev. of Voice Only Alter's Radius of Gyration(incoming activity) & 0.71&St. Dev. of the Mobile Money Alter's Outgoing SMS Network Size&	0.75                                \\ \hline \hline
	\end{tabular}
	\caption{\textbf{Top Features (tested individually).}  Individual features that are most predictive of churn. The ranked list of features is determined by individually assessing the ability of each feature to predict adoption, absent other features.\label{tab:features1}}
\end{table*}

==> tabs/uncond_features_pak.tex <==
\begin{table*}[tb]
	\centering
	\begin{tabular}{l*{4}{c}}
		\hline
		\textbf{Registered Mobile Money Feature}& \textbf{AUC}&\textbf{Active Mobile Money Feature}& \textbf{AUC} \\ \hline
		%1
		
		Ego's outgoing SMS Network Diversity&	0.58&Ego's outgoing SMS network diversity & 0.61 \\ 
		%2
		Average of Mobile Money Alter's  distance between A and B party&	0.58&Ego's Number of days with incoming SMS &0.60                               \\ 
		%3
		Std. Dev. of Mobile Money Alter's Location Diversity	&0.58&Ego's Network Diversity outgoing SMS and Voice& 0.59                             \\ 
		%4
		Std. Dev of Average Distance between A and B party for Mobile Money Alter	&0.58&Ego's Network Diversity Outgoing Voice & 0.58 \\  
		%5
		Standard Dev of Unique Days with activity for Mobile Money Alter &0.58&Ego's Network Diversity Voice & 0.58\\
		%6
		Average Distance between A and B party for Voice Communication for Mobile Money Alter&	0.58&Ego's SMS Network Diversity  & 0.58\\ 
		%7
		Standard Deviation of the Mobile Money Alter's Unique Receiving Locations	&0.58&Ego's Number of Days with SMS    & 0.58\\ 
		%8
		Standard Deviation of the Mobile Money Alter's Unique Receiving &	0.58&Ego's active days & 0.58\\ 
		%9
		Average Location Diversity for Mobile Money Alter	&0.58&Ego's number of days with incoming SMS  & 0.58\\
		%10
		Standard Dev. of the Unique Days with Voice Activity for Mobile Money Alter	&0.58&Ego's Average Distance between SMS parties  & 0.58\\ 
		\hline \hline
	\end{tabular}
	\caption{\textbf{Top Features (tested individually).}  Individual features that are most predictive of churn. The ranked list of features is determined by individually assessing the ability of each feature to predict adoption, absent other features.\label{tab:features1}}
\end{table*}

==> tabs/uncond_features_zambia.tex <==
\begin{table*}[tb]
	\centering
	\begin{tabular}{l*{4}{c}}
		\hline
		\textbf{Registered Mobile Money Feature}& \textbf{AUC}&\textbf{Active Mobile Money Feature}& \textbf{AUC} \\ \hline
		%1
		Ego's outgoing SMS Network Diversity&	0.58&Ego's outgoing SMS network diversity & 0.61 \\ 
		%2
		Average of Mobile Money Alter's  distance between A and B party&	0.58&Ego's Number of days with incoming SMS &0.60                               \\ 
		%3
		Std. Dev. of Mobile Money Alter's Location Diversity	&0.58&Ego's Network Diversity outgoing SMS and Voice& 0.59                             \\ 
		%4
		Std. Dev of Average Distance between A and B party for Mobile Money Alter	&0.58&Ego's Network Diversity Outgoing Voice & 0.58 \\  
		%5
		Standard Dev of Unique Days with activity for Mobile Money Alter &0.58&Ego's Network Diversity Voice & 0.58\\
		%6
		Average Distance between A and B party for Voice Communication for Mobile Money Alter&	0.58&Ego's SMS Network Diversity  & 0.58\\ 
		%7
		Standard Deviation of the Mobile Money Alter's Unique Receiving Locations	&0.58&Ego's Number of Days with SMS    & 0.58\\ 
		%8
		Standard Deviation of the Mobile Money Alter's Unique Receiving &	0.58&Ego's active days & 0.58\\ 
		%9
		Average Location Diversity for Mobile Money Alter	&0.58&Ego's number of days with incoming SMS  & 0.58\\
		%10
		Standard Dev. of the Unique Days with Voice Activity for Mobile Money Alter	&0.58&Ego's Average Distance between SMS parties  & 0.58\\ \hline \hline
	\end{tabular}
	\caption{\textbf{Top Features (tested individually).}  Individual features that are most predictive of churn. The ranked list of features is determined by individually assessing the ability of each feature to predict adoption, absent other features.\label{tab:features1}}
\end{table*}
